TwinLab: a framework for data-efficient training of non-intrusive reduced-order models for digital twins

Purpose: Simulation-based digital twins represent an effort to provide high-accuracy real-time insights into operational physical processes. However, the computation time of many multi-physical simulation models is far from real-time. It might even exceed sensible time frames to produce sufficient data for training data-driven reduced-order models. This study presents TwinLab, a framework for data-efficient, yet accurate training of neural-ODE type reduced-order models with only two data sets. Design/methodology/approach: Correlations between test errors of reduced-order models and distinct features of corresponding training data are investigated. Having found the single best data sets for training, a second data set is sought with the help of similarity and error measures to enrich the training process effectively. Findings: Adding a suitable second training data set in the training process reduces the test error by up to 49% compared to the best base reduced-order model trained only with one data set. Such a second training data set should at least yield a good reduced-order model on its own and exhibit higher levels of dissimilarity to the base training data set regarding the respective excitation signal. Moreover, the base reduced-order model should have elevated test errors on the second data set. The relative error of the time series ranges from 0.18% to 0.49%. Prediction speed-ups of up to a factor of 36,000 are observed. Originality: The proposed computational framework facilitates the automated, data-efficient extraction of non-intrusive reduced-order models for digital twins from existing simulation models, independent of the simulation software.

==> fig/03DynROMprinciple.tex <==
\begin{tikzpicture}[scale=0.15,declare function={a=8;b=4;c=2.5;s=5;}]
		\coordinate (A) at (0,0);
		\coordinate (B) at ($(A)-(13.5,5)-(s,0)$);
		\coordinate (C) at ($(A)-(a,0)-(s,0)$);
		\coordinate (D) at ($(C)-(0.1,0)$);
		\coordinate (TA) at ($(-0.45,2)-(s,0)$);
		\coordinate (TB) at ($(-0.45,3.99)-(s,0)$);
		\coordinate (TC) at ($(-0.45,0)-(s,0)$);
		\coordinate (N) at ($(A)+(50,20.58)$);
		
\draw[scale=1,fill=white, draw=black, thick] (B) rectangle +(27,25); 		
 \node[inner sep=0pt,anchor=south] at ($(B)+(13.5,25.5)$)   {Full-order model}; 
 
  \draw[scale=1, domain=0:180, smooth, variable=\x, black,draw=none, thick,dashed, fill=mygrey] plot ({a*cos(\x)-5}, {(b*sin(\x)});
  \draw[scale=1.0, domain=-1.5:181.5, smooth, variable=\x, black, thick] plot ({1.0*a*cos(\x)-5}, {(1.0*b*sin(\x)});
    \draw[thick] (D) -- +(2.02*a,0);	
    
    \draw[scale=1, domain=0:180, smooth, variable=\x, black,draw=none, thick,dashed, fill=mygrey] plot ({a*cos(\x)-5}, {(b*sin(\x)+10});
  \draw[scale=1.0, domain=-1.5:181.5, smooth, variable=\x, black, thick] plot ({1.0*a*cos(\x)-5}, {(1.0*b*sin(\x)+10});
    \draw[thick] ($(D)+(0,10)$) -- +(2.02*a,0);	  
 
 \draw[{Circle[open]}-latex] (TA) -- +($(17.5,0)+(s,0)$); %node[right] {$T_\text{A}$};	
 \draw[{Circle[open]}-latex](TB) -- +($(17.5,0)+(s,0)$); %node[right] {$T_\text{B}$};	
\draw[{Circle[open]}-latex] (TC) -- +($(17.5,0)+(s,0)$); %node[right] {$M_\text{db}$};	
% \node[rectangle, font=\large] at ($TA+(22,0)$)  {$=$};
% \node[right,rotate=0,anchor=west] at ($(TA)+(24,0)$)   {$= [T_{\text{A},1}, \dots, T_{\text{A},N} ]$};  
  \node[right,rotate=0,anchor=west] (E) at ($(TA)+(17.5,0)+(s,0)$)   {$  \begin{bmatrix}T_{\text{B},1}, \dots, T_{\text{B},N} \\ T_{\text{A},1}, \dots, T_{\text{A},N} \\ T_{\text{C},1}, \dots, T_{\text{C},N} \end{bmatrix} = \vect{\disphat[1.0mu]{Y}} $};  %\left[  \right] 
  % \\ M_{\text{db},1}, \dots, M_{\text{db},N}



%  \node[right,rotate=0,anchor=west] at ($(TB)+(24,0)$)  {$= [T_{\text{B},1}, \dots, T_{\text{B},N} ]$};   
%  \node[right,rotate=0,anchor=west] at ($(A)+(23.55,0)$)   {$= [M_{\text{db},1}, \dots, M_{\text{db},N} ]$}; 
  
  \draw[latex-] ($(13.55,8)-(s,0)$) -- +($(4.5,0)+(s,0)$) node[right] {$[T_{\text{oven},1}, \dots, T_{\text{oven},N}] = \vect{\disphat{G}}$};
   \draw[latex-] ($(A)+(50,0)+(0,8)$) -- +(-8.55,0);
%   \node[right,rotate=0,anchor=west] at ($(0,8)+(23.55,0)$)   {$= $};  
   
\draw[scale=1,fill=white, draw=black, thick, anchor=center] (N) rectangle +(27,-25); 	
 \node[inner sep=0pt,anchor=south] at ($(N)+(13.5,0.5)$)   {Reduced-order model}; 
 
\node[inner sep=0pt,anchor=north west] at ($(N)+(0.5,-0.5)$)
    {\includegraphics[width=.22\textwidth]{../tiks/RNN/rom-concept-down.pdf}};   
    
 \node[inner sep=0pt,anchor=west] at ($(N)+(2,-22)$)   
   {$\frac{\partial}{\partial t} \begin{bmatrix} \vect{X} \\ \vect{I} \end{bmatrix} = \vect{f} \left( \begin{bmatrix} \vect{X}\\ \vect{I}\end{bmatrix}, G,\vect{X}_0 \right)$};
      
    
      \draw[-latex] ($(N)+(0,-17.8)$) -- +(-7.3,0) node[left]{$\overset{!}{\approx} \vect{\disphat{X}} $};
%  \coordinate (Int) at (0,-.11);
%  \draw[latex-, font=\large] (-2.0,0) -- +(-1*0.7,1.5*0.7) node[above] {$\Gamma_\text{porous}$};
  
  
%  \draw[latex-, font=\large] (Int) -- +(0.9*1,-1.5*0.9) node[below] {$\Gamma_\text{air, interf}$};
%  \draw[latex-] (6.2,-5) -- +(-1*0.9,1.5*0.9) node[above] {$\Gamma_\text{air}$};;
  
%  \node[rectangle, font=\large] (Por) at (2.3,2) {$\Omega_\text{porous}$};
%   \node[rectangle, font=\large] (Flu) at (10,7) {$\Omega_\text{air}$};
\end{tikzpicture}
%
%\begin{tikzpicture}[scale=0.15,declare function={a=8;b=4;c=2.5;}]
%		\coordinate (A) at (0,0);
%		\coordinate (B) at ($(A)-(12.5,5)$);
%		\coordinate (C) at ($(A)-(a,0)$);
%		\coordinate (D) at ($(C)-(0.1,0)$);
%		\coordinate (TA) at (-0.45,2);
%		\coordinate (TB) at (-0.45,3.99);
%		\coordinate (TC) at (-0.45,0);
%		\coordinate (N) at ($(A)+(50,20.58)$);
%		
%\draw[scale=1,fill=white, draw=black, thick] (B) rectangle +(25,15); 		
% \node[inner sep=0pt,anchor=south] at ($(B)+(12.5,15.5)$)   {Full-order model}; 
% 
%  \draw[scale=1, domain=0:180, smooth, variable=\x, black,draw=none, thick,dashed, fill=mygrey] plot ({a*cos(\x)}, {(b*sin(\x)});
%%\draw[thick, dashed] (C) -- +(2*a,0);	
%
%  \draw[scale=1.0, domain=-1.5:181.5, smooth, variable=\x, black, thick] plot ({1.0*a*cos(\x)}, {(1.0*b*sin(\x)});
%    \draw[thick] (D) -- +(2.02*a,0);	
% 
% \draw[{Circle[open]}-latex] (TA) -- +(17.5,0); %node[right] {$T_\text{A}$};	
% \draw[{Circle[open]}-latex](TB) -- +(17.5,0); %node[right] {$T_\text{B}$};	
%\draw[{Circle[open]}-latex] (TC) -- +(17.5,0); %node[right] {$M_\text{db}$};	
%% \node[rectangle, font=\large] at ($TA+(22,0)$)  {$=$};
%% \node[right,rotate=0,anchor=west] at ($(TA)+(24,0)$)   {$= [T_{\text{A},1}, \dots, T_{\text{A},N} ]$};  
%  \node[right,rotate=0,anchor=west] (E) at ($(TA)+(17.5,0)$)   {$  \begin{bmatrix}T_{\text{B},1}, \dots, T_{\text{B},N} \\ T_{\text{A},1}, \dots, T_{\text{A},N} \\ T_{\text{C},1}, \dots, T_{\text{C},N} \end{bmatrix} = \vect{\disphat[1.0mu]{Y}} $};  %\left[  \right] 
%  % \\ M_{\text{db},1}, \dots, M_{\text{db},N}
%
%
%
%%  \node[right,rotate=0,anchor=west] at ($(TB)+(24,0)$)  {$= [T_{\text{B},1}, \dots, T_{\text{B},N} ]$};   
%%  \node[right,rotate=0,anchor=west] at ($(A)+(23.55,0)$)   {$= [M_{\text{db},1}, \dots, M_{\text{db},N} ]$}; 
%  
%  \draw[latex-] (12.5,8) -- +(4.55,0) node[right] {$[T_{\text{oven},1}, \dots, T_{\text{oven},N}] = \vect{\disphat{G}}$};
%   \draw[latex-] ($(A)+(50,0)+(0,8)$) -- +(-8.55,0);
%%   \node[right,rotate=0,anchor=west] at ($(0,8)+(23.55,0)$)   {$= $};  
%   
%\draw[scale=1,fill=white, draw=black, thick, anchor=center] (N) rectangle +(27,-25); 	
% \node[inner sep=0pt,anchor=south] at ($(N)+(13.5,0.5)$)   {Reduced-order model}; 
% 
%\node[inner sep=0pt,anchor=north west] at ($(N)+(0.5,-0.5)$)
%    {\includegraphics[width=.24\textwidth]{../tiks/RNN/rom-concept-down.pdf}};   
%    
% \node[inner sep=0pt,anchor=west] at ($(N)+(2,-22)$)   
%   {$\frac{\partial}{\partial t} \begin{bmatrix} \vect{X} \\ \vect{I} \end{bmatrix} = f \left( \begin{bmatrix} \vect{X}\\ \vect{I}\end{bmatrix}, G,\vect{X}_0 \right)$};
%      
%    
%      \draw[-latex] ($(N)+(0,-17.8)$) -- +(-7.3,0) node[left]{$\overset{!}{\approx} \vect{\disphat{X}} $};
%%  \coordinate (Int) at (0,-.11);
%%  \draw[latex-, font=\large] (-2.0,0) -- +(-1*0.7,1.5*0.7) node[above] {$\Gamma_\text{porous}$};
%  
%  
%%  \draw[latex-, font=\large] (Int) -- +(0.9*1,-1.5*0.9) node[below] {$\Gamma_\text{air, interf}$};
%%  \draw[latex-] (6.2,-5) -- +(-1*0.9,1.5*0.9) node[above] {$\Gamma_\text{air}$};;
%  
%%  \node[rectangle, font=\large] (Por) at (2.3,2) {$\Omega_\text{porous}$};
%%   \node[rectangle, font=\large] (Flu) at (10,7) {$\Omega_\text{air}$};
%\end{tikzpicture}

==> tiks/ROM-signal-evals/APRBSEqual15-RMSE-stdTb-Show-a4.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor2}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor3}{rgb}{0.65098,0.00000,0.51765}%
%
\begin{tikzpicture}

\begin{axis}[%
xmin=0,
xmax=10,
xlabel style={font=\color{white!15!black}},
xlabel={RMSE},
ymin=5,
ymax=35,
ylabel style={font=\color{white!15!black}},
ylabel={stdTb},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Eval on:APRBSEqual15},
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
width = \fwidth, 
 height = \fheight 
]
%\addplot [color=black, only marks, mark=*, mark options={solid, black}]
%  table[]{../tiks/ROM-signal-evals/APRBSEqual15-RMSE-stdTb-Show-a4-1.tsv};
%\addlegendentry{Data}

\addplot [color=black]
  table[]{../tiks/ROM-signal-evals/APRBSEqual15-RMSE-stdTb-Show-a4-2.tsv};
\addlegendentry{Fit}

\addplot [color=black, dashed]
  table[]{../tiks/ROM-signal-evals/APRBSEqual15-RMSE-stdTb-Show-a4-3.tsv};
\addlegendentry{$\text{Prediction p \textgreater{} 0.95}$}

\addplot [color=black, dashed, forget plot]
  table[]{../tiks/ROM-signal-evals/APRBSEqual15-RMSE-stdTb-Show-a4-4.tsv};
\addplot [color=mycolor1, only marks, mark=diamond*, mark options={solid, fill=black, black}]
  table[]{../tiks/ROM-signal-evals/APRBSEqual15-RMSE-stdTb-Show-a4-5.tsv};
\addlegendentry{APRBS}

\addplot [color=mycolor2, only marks, mark=diamond*, mark options={solid, fill=mycolor3, mycolor3}]
  table[]{../tiks/ROM-signal-evals/APRBSEqual15-RMSE-stdTb-Show-a4-6.tsv};
\addlegendentry{Best 5 APRBS}

%\node[below right, align=left]
%at (axis cs:3.446,21.92) {282-a4};
%\node[below right, align=left]
%at (axis cs:1.822,26.276) {286-a4};
%\node[below right, align=left]
%at (axis cs:2.176,25.02) {293-a4};
%\node[below right, align=left]
%at (axis cs:1.349,26.396) {298-a4};
%\node[below right, align=left]
%at (axis cs:3.363,21.483) {302-a4};
%\node[below right, align=left]
%at (axis cs:3.855,22.105) {303-a4};
%\node[below right, align=left]
%at (axis cs:1.125,31.75) {312-a4};
%\node[below right, align=left]
%at (axis cs:7.538,14.39) {322-a4};
%\node[below right, align=left]
%at (axis cs:2.456,23.518) {328-a4};
%\node[below right, align=left]
%at (axis cs:2.612,27.316) {337-a4};
%\node[below right, align=left]
%at (axis cs:4.571,19.975) {341-a4};
%\node[below right, align=left]
%at (axis cs:5.118,22.547) {342-a4};
%\node[below right, align=left]
%at (axis cs:9.62,17.592) {351-a4};
%\node[below right, align=left]
%at (axis cs:3.26,19.57) {355-a4};
%\node[below right, align=left]
%at (axis cs:1.262,25.243) {360-a4};
%\node[below right, align=left]
%at (axis cs:3.078,19.852) {369-a4};
%\node[below right, align=left]
%at (axis cs:6.429,14.477) {371-a4};
%\node[below right, align=left]
%at (axis cs:1.493,29.802) {378-a4};
%\node[below right, align=left]
%at (axis cs:1.898,25.178) {383-a4};
%\node[below right, align=left]
%at (axis cs:1.547,24.666) {400-a4};
%\node[below right, align=left]
%at (axis cs:2.391,22.015) {404-a4};
%\node[below right, align=left]
%at (axis cs:2.217,26.678) {425-a4};
%\node[below right, align=left]
%at (axis cs:3.911,20.146) {437-a4};
%\node[below right, align=left]
%at (axis cs:1.778,26.521) {473-a4};
%\node[below right, align=left]
%at (axis cs:5.744,17.115) {479-a4};
%\node[below right, align=left]
%at (axis cs:2.098,25.89) {485-a4};
%\node[below right, align=left]
%at (axis cs:4.757,18.388) {510-a4};
%\node[below right, align=left]
%at (axis cs:1.79,22.196) {514-a4};
%\node[below right, align=left]
%at (axis cs:4.413,18.51) {517-a4};
%\node[below right, align=left]
%at (axis cs:4.405,17.181) {520-a4};
%\node[below right, align=left]
%at (axis cs:2.866,26.374) {534-a4};
%\node[below right, align=left]
%at (axis cs:5.413,23.037) {538-a4};
%\node[below right, align=left]
%at (axis cs:1.068,22.552) {553-a4};
%\node[below right, align=left]
%at (axis cs:8.541,19.597) {555-a4};
%\node[below right, align=left]
%at (axis cs:1.868,30.064) {559-a4};
%\node[below right, align=left]
%at (axis cs:4.744,19.355) {572-a4};
%\node[below right, align=left]
%at (axis cs:3.206,22.614) {590-a4};
%\node[below right, align=left]
%at (axis cs:1.443,24.279) {595-a4};
%\node[below right, align=left]
%at (axis cs:4.05,22.74) {622-a4};
%\node[below right, align=left]
%at (axis cs:1.2,26.132) {625-a4};
%\node[below right, align=left]
%at (axis cs:6.6,14.026) {637-a4};
%\node[below right, align=left]
%at (axis cs:2.664,22.93) {678-a4};
%\node[below right, align=left]
%at (axis cs:2.507,23.806) {683-a4};
%\node[below right, align=left]
%at (axis cs:2.757,21.611) {699-a4};
%\node[below right, align=left]
%at (axis cs:1.726,28.344) {703-a4};
%\node[below right, align=left]
%at (axis cs:7.643,14.624) {706-a4};
%\node[below right, align=left]
%at (axis cs:2.393,25.87) {707-a4};
%\node[below right, align=left]
%at (axis cs:2.512,20.159) {712-a4};
%\node[below right, align=left]
%at (axis cs:2.009,24.955) {727-a4};
%\node[below right, align=left]
%at (axis cs:3.813,26.884) {731-a4};
%\node[below right, align=left]
%at (axis cs:6.074,21.87) {732-a4};
%\node[below right, align=left]
%at (axis cs:3.48,18.707) {737-a4};
%\node[below right, align=left]
%at (axis cs:1.071,26.165) {745-a4};
%\node[below right, align=left]
%at (axis cs:3.754,20.364) {751-a4};
%\node[below right, align=left]
%at (axis cs:1.226,25.359) {762-a4};
\legend{};
\end{axis}

\begin{axis}[%
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={only marks},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black},
width = \fwidth, 
 height = \fheight 
]
\node[fill=white, below right, align=left, draw=black]
at (rel axis cs:0.02,0.071) {R = -0.76198};
\end{axis}
\end{tikzpicture}%
